Symplectic Lie groups and nilmanifolds associated with acyclic quivers

We give combinatorial criteria for the existence of left-invariant symplectic forms on the positive and full path Lie groups of finite acyclic quivers. For the nilpotent positive path Lie groups, the criterion also determines whether their compact quotients admit symplectic forms and forces the nilpotency step to be at most three. For the completely solvable full path Lie groups, we give a direct combinatorial criterion and an equivalent recursive criterion. In the symplectic case, the recursive procedure is realized by successive Hamiltonian reductions ending at an abelian symplectic Lie group. We characterize the existence of Lagrangian normal subgroups for a given form in both families, with applications to Lagrangian torus fibrations of compact nilmanifolds. We also describe the cohomology rings of the compact symplectic nilmanifolds and determine all Lefschetz ranks.

==> symplectic_computations/reference/computation_excerpts.tex <==
% Exact statement excerpts from symplectic_quivers.tex.
% For source comparison only; this is not a standalone LaTeX document.

% def:activedata (4.6)
\begin{definition}\label{def:activedata}
We call the predecessors and successors of active families
boundary arrows.
The set of predecessors and the set of successors are disjoint,
since an arrow belonging to both would give a path
of length at least four.
The active-family graph $G_A(Q)$ is the bipartite graph with these two sets
as its parts, with one edge joining the predecessor
and successor of each active family.

In each connected component of $\GR$ isomorphic to
$K_{1,\ell}$, choose a central vertex, choosing the boundary
arrow if the component contains one.
This is possible by Lemma~\ref{lem:residualstars}.
Together with all isolated vertices of $\GR$,
denote the chosen vertices by $a_1,\cdots,a_b$.
We call $a_1,\cdots,a_b$ the chosen residual arrows.
Every boundary arrow occurs among them.
If $a_i$ belongs to a component $K_{1,\ell}$,
let $\ell_i=\ell$; if $a_i$ is isolated, let $\ell_i=0$.
Let $c_\square$ be the number of components isomorphic
to $K_{2,2}$.

For each active family with predecessor $a_i$ and
successor $a_j$, let $r_{ij}=r_{ji}$ be the number of its active arrows.
Let $r_{ii}=0$, and let $r_{ij}=0$ if no active family
has $a_i,a_j$ as its predecessor and successor
in either order.
Sums over $\{i,j\}$ are taken over unordered pairs
of distinct indices, so each active family is counted once.
\end{definition}

% def:inversegraph (4.7)
\begin{definition}\label{def:inversegraph}
The projection $\nq=K\oplus H_R\to H_R$ restricts
to an isomorphism from $K^{\perp_\omega}$ onto $H_R$.
Use this isomorphism to transfer
$\omega|_{K^{\perp_\omega}}$ to a form $\omega_R$ on $H_R$.
For a boundary arrow $a$, let $a^*$ be the element
of the basis of $H_R^*$ dual to the path basis
that corresponds to $a$.
The inverse form $\omega_R^{-1}$ is the alternating form
on $H_R^*$ whose matrix in the dual basis is the inverse
of the matrix of $\omega_R$.
The inverse form graph $F_\omega$ has the boundary arrows
as vertices, with $a,c$ adjacent exactly when
$\omega_R^{-1}(a^*,c^*)\ne0$.
\end{definition}

% thm:nilidealcriterion (4.8)
\begin{theorem}\label{thm:nilidealcriterion}
The symplectic Lie group $(N_Q,\Omega)$ has a connected closed
Lagrangian normal subgroup if and only if $G_A(Q)$ has a
vertex cover which is independent in $F_\omega$.
If $\omega$ is rational and $G_A(Q)$ has a vertex cover
which is independent in $F_\omega$, then $(N_Q,\Omega)$
has a rational connected closed Lagrangian normal subgroup.
\end{theorem}

% ex:twenty (4.14)
\begin{example}\label{ex:twenty}
Among the Lie algebras $\nq$ associated with finite acyclic
quivers, the minimum dimension admitting a symplectic form
with no Lagrangian ideal is $20$.

This minimum is attained by the following quiver $Q$.
\begin{center}
\begin{tikzcd}[column sep=large, row sep=large]
& u_1
  \arrow[r, shift left=1, "b_{11}"]
  \arrow[r, shift right=1, "b_{12}"']
& v_1 \arrow[dr, "c_1"] & \\
s \arrow[ur, "a_1"] \arrow[dr, "a_2"']
& & & t \\
& u_2
  \arrow[r, shift left=1, "b_{21}"]
  \arrow[r, shift right=1, "b_{22}"']
& v_2 \arrow[ur, "c_2"'] &
\end{tikzcd}
\end{center}
Here $\dim\nq=20$.
For $i=1,2$, let
$K_i=\Span\{b_{ij},a_ib_{ij},b_{ij}c_i,a_ib_{ij}c_i
\mid j=1,2\}$.
Let $\omega_K$ be the form constructed before
Lemma~\ref{lem:coreformclosed}, taking
$J=\begin{psmallmatrix}0&1\\-1&0\end{psmallmatrix}$
for each of the two active families.
 Let $\theta_1,\cdots,\theta_4$ be the basis
of $H_R^*$ dual to $(a_1,c_1,a_2,c_2)$.
Define
$\omega_0=\omega_K+\theta_1\wedge\theta_2+
\theta_3\wedge\theta_4$ and
$\omega_1=\omega_K+\sum_{i<j}\theta_i\wedge\theta_j$.
Both are symplectic forms with integer coefficients
in the path basis.

For $i=0,1$, let $\Omega_i$ be the left-invariant
extension of $\omega_i$ to $N_Q$.
Let $\overline\Omega_i$ be the form on
$M_Q=\Gamma_Q\backslash N_Q$ induced by $\Omega_i$.
Then $(N_Q,\Omega_0)$ has a rational connected closed
Lagrangian normal subgroup, whereas $(N_Q,\Omega_1)$
has no connected closed Lagrangian normal subgroup.
Consequently, $(M_Q,\overline\Omega_0)$ admits a
Lagrangian torus fibration induced by a rational normal
subgroup, with ten-dimensional fibers, whereas
$(M_Q,\overline\Omega_1)$ admits no such fibration.


\end{example}

% thm:fullisotropicrank (6.7)
\begin{theorem}\label{thm:fullisotropicrank}
Write $\rank(\beta|_{\mathfrak z_Q})=2r$.
The maximum dimension of a connected closed isotropic normal
subgroup of $(S_Q,\Omega)$ is $a(Q)+c(Q)-r$.
Consequently, $(S_Q,\Omega)$ has a connected closed Lagrangian
normal subgroup exactly when
$a(Q)+c(Q)-r=\tfrac12(n(Q)+m(Q))$.
Equivalently, the symplectic rank is
$\sigma(\sq,\omega)=a(Q)+c(Q)-r$.
For connected $Q$, this maximum and the existence of such a
Lagrangian normal subgroup are independent of $\Omega$.
\end{theorem}

% rem:cutalgorithm (6.8)
\begin{remark}\label{rem:cutalgorithm}
The number $a(Q)$ can be computed from arrow weights.
Let $p(v)$ and $q(v)$ count the paths ending and starting
at $v$, including the trivial path.
Compute $p(v)$ in a topological order and $q(v)$
in the reverse topological order.
Assign each arrow from $u$ to $v$ the weight $p(u)q(v)$.
Since every path crossing a downward closed set $D$
contains exactly one arrow leaving $D$, $a(Q)$ is the maximum
total weight of arrows leaving such a set.
On each tree, this maximum is computed recursively by
considering whether each vertex belongs to $D$,
with no arrow allowed to enter $D$ from outside.
\end{remark}

% ex:triangularrank (6.9)
\begin{example}\label{ex:triangularrank}

The existence of a Lagrangian subgroup does not imply
the existence of a Lagrangian normal subgroup.
For the Lie groups $T_q^+$, we show more precisely that the
difference between the dimension of a Lagrangian subgroup
and the largest possible dimension of a connected closed
isotropic normal subgroup is unbounded as $q$ varies.


For the directed path $A_q$, every downward closed set
consists of the first $j$ vertices and is crossed by
$j(q-j)$ paths.
Hence $a(A_q)=\lfloor q^2/4\rfloor$.
Since $A_q$ is connected, Theorem~\ref{thm:fullisotropicrank}
gives $\sigma(\mathfrak t_q,\omega)=\lfloor q^2/4\rfloor+1$
for every symplectic form $\omega$, whenever
$q\equiv0,3\pmod4$.
Thus the difference between the dimension of a Lagrangian
subgroup and the maximum dimension of an isotropic normal
subgroup is
$\Delta_q=\frac{q(q+1)}4-\lfloor q^2/4\rfloor-1$.
In particular, $\Delta_{4k}=k-1$ for $k\ge1$ and
$\Delta_{4k+3}=k$ for $k\ge0$.

For $q=7$, the group $T_7^+$ has dimension $28$,
whereas $\sigma(\mathfrak t_7,\omega)=13$.
By Theorem~\ref{thm:lagrangiansubgroup}, every left-invariant
symplectic form on $T_7^+$ admits a connected closed
Lagrangian subgroup of dimension $14$.
However, no such subgroup is normal.
Equivalently, Lagrangian subalgebras exist but Lagrangian
ideals do not.
An explicit symplectic form is $\omega=\beta+d\lambda$, where
$\lambda(E_{17})=\lambda(E_{26})=\lambda(E_{35})=1$,
$\lambda$ vanishes on all other non-trivial paths, and
$\beta=E_{11}^*\wedge E_{22}^*+E_{33}^*\wedge E_{44}^*$.
Its matrix has determinant one by the construction in
Proposition~\ref{prop:integral}.

\end{example}

% prop:moduledecomposition (7.1)
\begin{proposition}\label{prop:moduledecomposition}
There is an isomorphism
$\nq\cong(\mathfrak a\ltimes V)\oplus
\mathfrak g_\square^{\oplus c_\square}$,
where $\mathfrak a=\Span\{a_1,\cdots,a_b\}$ and $V$ are
abelian, and $\mathfrak g_\square$ is the Lie algebra of
$K_{2,2}$.
The $\mathfrak a$-action on $V^*$ extends to
$\mathfrak{sl}_2^{\oplus b}$,
with
\begin{equation*}
 V^*\cong\bigoplus_i S_i^{\oplus\ell_i}
 \ \oplus\!\bigoplus_{\{i,j\}}(S_i\otimes S_j)^{\oplus r_{ij}}.
\end{equation*}
Under this identification, $a_i$ acts as the raising operator
$E_i$, where
$E_i$ has $\begin{psmallmatrix}0&1\\0&0\end{psmallmatrix}$
in the $i$th summand of $\mathfrak{sl}_2^{\oplus b}$
and zero in all other summands.
\end{proposition}

% thm:betti (7.2)
\begin{theorem}\label{thm:betti}
Since $\nq$ is symplectic, every compact quotient
$\Gamma\backslash N_Q$ has Poincar\'e polynomial
$\operatorname{Poin}_Q(z)=(1+z)^b
\bigl(\sum_q \kappa_qz^q\bigr)P_\square(z)^{c_\square}$.
\end{theorem}

% prop:ringmodel (7.3)
\begin{proposition}\label{prop:ringmodel}
There is an isomorphism of graded algebras
$H^*(\mathfrak a\ltimes V)\cong(\mathcal E_Q,\star)$,
where $\mathcal E_Q=\bigoplus_I\theta_I\operatorname{im}P_I$
is the space of representatives defined by the projections $P_I$.
For $f\in\operatorname{im}P_I\cap\Lambda^qV^*$
and $g\in\operatorname{im}P_J$, the product is defined by
\begin{equation*}
 (\theta_If)\star(\theta_Jg)
 =(-1)^{q|J|}\theta_I\wedge\theta_J\wedge
 P_{I\cup J}(f\wedge g).
\end{equation*}
It is zero if $I\cap J\ne\varnothing$.
Consequently,
$H^*(M)\cong(\mathcal E_Q,\star)\otimes
H^*(\mathfrak g_\square)^{\otimes c_\square}$
as graded algebras.
\end{proposition}

% thm:firstlefschetz (7.4)
\begin{theorem}\label{thm:firstlefschetz}
Suppose $\dim M=2d>0$, and let $\omega$ be
a symplectic form on $M$.
Then $b_1(M)=|Q_1|$ and
$\rank L_\omega^{d-1}=|Q_1|-\nu(Q)$ on $H^1(M)$.
Equivalently, this rank is the number of tree components
of $\GR$, including isolated vertices.
Let $\eta$ be a closed two-form on $\nq$ whose induced
form on $M$ represents $[\omega]$.
Then $\ker L_\omega^{d-1}
=\{[\iota_z\eta]\mid z\in Z(\nq)\cap[\nq,\nq]\}$,
where $(\iota_z\eta)(x)=\eta(z,x)$ for $x\in\nq$.

\end{theorem}

% lem:starnormal (7.6)
\begin{lemma}\label{lem:starnormal}
Each matrix $B^{(i)}$ is symmetric and has corank at most one.
Let $D=\{i\mid\dim\ker B^{(i)}=1\}$.
For $i\in D$, let $u_i$ span the radical of $B^{(i)}$
in $\Span\{u_{i1},\cdots,u_{i\ell_i}\}$ and let $z_i=[a_i,u_i]$.
There is a Lie algebra automorphism $\Phi$ such that,
after replacing $\omega$ by $\Phi^*\omega$, the following
assertions hold:
$\nq=(\mathfrak h\ltimes W)\oplus
\mathfrak g_\square^{\oplus c_\square}$ is a symplectic
direct sum, where
$\mathfrak h=
\bigoplus_{i\in D}\mathfrak h_3(a_i,u_i,z_i)
\oplus\bigoplus_{i\notin D}\mathbb R a_i$,
each $\mathfrak h_3(a_i,u_i,z_i)$ has $[a_i,u_i]=z_i$
as its only nonzero bracket, and
$[W,W]=[u_i,W]=[z_i,W]=0$ for $i\in D$.
Here $W$ is the abelian ideal obtained from $K$ and the
spaces $U_i'\oplus[a_i,U_i']$, where $U_i'$ is a complement
to the radical of $B^{(i)}$ in the span of the $u_{ij}$.
Moreover,
\begin{equation*}
W^*\cong
\bigoplus_i S_i^{\oplus(\ell_i-\mathbf1_D(i))}
\oplus
\bigoplus_{\{i,j\}}(S_i\otimes S_j)^{\oplus r_{ij}}.
\end{equation*}
The restriction of $\omega$ to $\mathfrak h\ltimes W$ is
$\Omega_W+\sum_{i\in D}\theta_i\wedge\zeta_i+\beta$,
where $\Omega_W=\omega|_W$ is nondegenerate,
$\theta_i=a_i^*$ and $\zeta_i=-z_i^*$, so
$d\zeta_i=\theta_i\wedge u_i^*$.
Let
$U=\Span\bigl(\{u_i\mid i\in D\}
\cup\{a_i\mid i\notin D\}\bigr)$.
Then $\beta\in\Lambda^2U^*$ is nondegenerate,
with $\Omega_W$ and $\beta$ extended by zero to the
other summands.
\end{lemma}

% lem:localcoefficients (7.7)
\begin{lemma}\label{lem:localcoefficients}
The graded vector spaces $H^*(\mathfrak h_3;V_p)$,
together with the operators $\mathsf U$ and $\mathsf T$,
are described by the following table.
All exterior generators have degree one.
\begin{center}
\begin{tabular}{ccl}
\toprule
$p$ & Graded space & Operators \\
\midrule
$0$ & $(\Lambda(\upsilon)\otimes J_2)
       \oplus\kk[1]\oplus\kk[2]$
 & $\mathsf U=\upsilon\wedge$, $\mathsf T$ acts on $J_2$ \\
$1$ & $\Lambda(\upsilon,v,w)$
 & $\mathsf U=\upsilon\wedge$, $\mathsf T=(\upsilon\wedge v)\wedge$ \\
$\ge2$ & $\Lambda(\upsilon,v,w)$
 & $\mathsf U=\upsilon\wedge$, $\mathsf T=0$ \\
\bottomrule
\end{tabular}
\end{center}
For $p=0$, both operators vanish on
$\kk[1]\oplus\kk[2]$.
For the one-dimensional abelian Lie algebra
$\kk a$, with $a$ acting on $V_p$ by the
raising operator, the cohomology
$H^*(\kk a;V_p)$ has dimension one
in each of degrees zero and one.
Multiplication by $[\theta]$ is nonzero
if and only if $p=0$.
\end{lemma}

% thm:allstrings (7.8)
\begin{theorem}\label{thm:allstrings}


All graded Lefschetz strings on $H^*(\nq)$ are obtained
as follows.
For each $0\le q\le d_W$ and
$\mathbf p\in\mathbb Z_{\ge0}^b$ with $c_{q,\mathbf p}>0$,
and for each $A\subseteq D_0$, perform the following steps.
\begin{enumerate}
\item Define
$S=A\cup D_2\cup O_0$, $
e=|A\cup D_1\cup D_2\cup O_0|
  +2|D_1\cup D_2|+|O_1|$, $
2r=2|D_1|+\rank\beta_S$, and $ 
 h=|D_0\setminus A|$.
\item Take the strings in Lemma~\ref{lem:stringrules}
for an exterior algebra on a space of dimension $e$
with an alternating form of rank $2r$.
Tensor them with $(q,d_W-q+1)$ and with $|A|$ copies
of $(0,2)$, using the tensor product rule in that lemma.
\item For each $0\le s\le h$, shift all starting degrees
by $h+s$ and multiply the multiplicities by
$c_{q,\mathbf p}\binom hs$.
\end{enumerate}
Collect the resulting strings over all $q,\mathbf p,A$.
This gives the graded Lefschetz strings on
$H^*(\mathfrak h\ltimes W)$.
Finally, tensor them with the Lefschetz strings of the
restricted symplectic form on each
$\mathfrak g_\square$ factor.
The resulting strings, counted with multiplicity,
are all graded Lefschetz strings on $H^*(\nq)$.

For $k,u\ge0$, each occurrence of a string $(a,\ell)$
contributes one to
$\rank(L_\omega^u:H^k\to H^{k+2u})$
if $k-a$ is nonnegative and even
and $(k-a)/2+u<\ell$, and contributes zero otherwise.

\end{theorem}

% ex:lefschetzvariation (7.10)
\begin{example}\label{ex:lefschetzvariation}

Consider the quiver
\begin{center}
\begin{tikzcd}[column sep=large, row sep=large]
s \arrow[r, "a"]
& u \arrow[r, shift left=1, "b_1"]
    \arrow[r, shift right=1, "b_2"']
    \arrow[d, "f"']
& v \arrow[r, "c"]
& t \\
& w & &
\end{tikzcd}
\end{center}
There are twelve non-trivial paths.
The ideal $K$ has basis
$b_i,ab_i,b_ic,ab_ic$ for $i=1,2$.
Let
$\Omega_K=(ab_1c)^*\wedge b_2^*
-(ab_2c)^*\wedge b_1^*
+(ab_2)^*\wedge(b_1c)^*
-(ab_1)^*\wedge(b_2c)^*$,
and define
$\omega_0=\Omega_K+a^*\wedge(af)^*+f^*\wedge c^*$
and
$\omega_1=\Omega_K+a^*\wedge(af)^*+f^*\wedge c^*
+f^*\wedge(af)^*$.
Both forms are closed and nondegenerate.

The residual graph $\GR$ consists of the edge
$\{a,f\}$ and the isolated vertex $c$.
Choose $a$ as the central vertex of the component
$K_{1,1}$ on $\{a,f\}$.
For $\omega_j$, the corresponding matrix is
$B_j=(\omega_j(af,f))$, where $j=0,1$.
Thus $B_0=(0)$ and $B_1=(-1)$ have corank one
and zero, respectively.
 Theorem~\ref{thm:allstrings} gives the following ranks of
$L^{6-k}:H^k\to H^{12-k}$.
\begin{center}
\begin{tabular}{c|rrrrr}
$k$ & $0$ & $1$ & $2$ & $3$ & $4$ \\
\hline
$\omega_0$ & $1$ & $2$ & $9$ & $30$ & $75$ \\
$\omega_1$ & $1$ & $2$ & $9$ & $32$ & $79$
\end{tabular}
\end{center}
Thus $\omega_0$ and $\omega_1$ induce the same
Lefschetz ranks on $H^1$ and $H^2$, but different ranks on
$H^3$ and $H^4$ of the same compact nilmanifold.


\end{example}

% prop:secondlefschetz (7.11)
\begin{proposition}\label{prop:secondlefschetz}
Suppose that $\GR$ has no edges and that at least one active
family exists. For the symplectic form $\omega=\omega_K(J)+\beta$,
the rank on $H^2$ is
\begin{equation*}
 \rank L_\omega^{N-2}
 =\binom b2+\sum_e\binom{r_e}{2}
 +2\sum_{\substack{e=\{i,j\}\\\Pi_{ij}\ne0}}r_e.
\end{equation*}
\end{proposition}

% prop:secondsupport (7.12)
\begin{proposition}\label{prop:secondsupport}
Under the assumptions of Proposition~\ref{prop:secondlefschetz},
for any $F\subseteq E(G_A(Q))$, there exists a
symplectic form $\omega=\omega_K(J)+\beta$ such that  
$\Pi_{ij}\ne0$ for $\{i,j\}\in F$ and
$\Pi_{ij}=0$ for $\{i,j\}\in E(G_A(Q))\setminus F$
if and only if
$K_b\setminus(E(G_A(Q))\setminus F)$
has a perfect matching.
\end{proposition}

% prop:secondextrema (7.13)
\begin{proposition}\label{prop:secondextrema}
Under the assumptions of Proposition~\ref{prop:secondlefschetz},
give the edges of $K_b$ weight $r_e$ on
$G_A(Q)$ and zero elsewhere. 
Let $w_{\min}$ be the minimum among the weights of all
perfect matchings of $K_b$, where the weight of a matching is the sum of the weights of its edges.
Then the minimum rank of $L_\omega^{N-2}$ on $H^2$ is
$\binom b2+\sum_e\binom{r_e}{2}+2w_{\min}$;
its maximum is
$\binom b2+\sum_e\binom{r_e}{2}+2\sum_e r_e$.
\end{proposition}

